Minimal $(D,D)$ conformal matter and generalizations of the van Diejen model

We consider supersymmetric surface defects in compactifications of the $6d$ minimal $(D_{N+3},D_{N+3})$ conformal matter theories on a punctured Riemann surface. For the case of $N=1$ such defects are introduced into the supersymmetric index computations by an action of the $BC_1\,(\sim A_1\sim C_1)$ van Diejen model. We (re)derive this fact using three different field theoretic descriptions of the four dimensional models. The three field theoretic descriptions are naturally associated with algebras $A_{N=1}$, $C_{N=1}$, and $(A_1)^{N=1}$. The indices of these $4d$ theories give rise to three different Kernel functions for the $BC_1$ van Diejen model. We then consider the generalizations with $N>1$. The operators introducing defects into the index computations are certain $A_{N}$, $C_N$, and $(A_1)^{N}$ generalizations of the van Diejen model. The three different generalizations are directly related to three different effective gauge theory descriptions one can obtain by compactifying the minimal $(D_{N+3},D_{N+3})$ conformal matter theories on a circle to five dimensions. We explicitly compute the operators for the $A_N$ case, and derive various properties these operators have to satisfy as a consequence of $4d$ dualities following from the geometric setup. In some cases we are able to verify these properties which in turn serve as checks of said dualities. As a by-product of our constructions we also discuss a simple Lagrangian description of a theory corresponding to compactification on a sphere with three maximal punctures of the minimal $(D_5,D_5)$ conformal matter and as consequence give explicit Lagrangian constructions of compactifications of this 6d SCFT on arbitrary Riemann surfaces.

==> sections/app_d4_trinion__Case_Conflict_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(2)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_10_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_11_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_12_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_13_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_14_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_15_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_16_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_17_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_1_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(2)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_2_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(2)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_3_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(2)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_4_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(2)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_5_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(2)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_6_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_7_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_8_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/app_d4_trinion__Case_Conflict_9_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Derivation of the $(D_5,D_5)$ trinion}
\label{app:D4:trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us discuss here the description for the sphere with two minimal and two maximal punctures that we have obtained  in the previous section and shown on the Figure \ref{pic:4pt:seib}.
The description  is  $\SU(N+3)$ SQCD in the middle of the conformal window with flip fields. The superpotentials correspond to triangles in the quiver and to certain baryonic operators: these are all the operators of R-charge two with vanishing charges for global symmetries. Note that although the triangle superpotentials are relevant the baryonic superpotentials are irrelevant for $N>1$. 

First the form of the theory after the sequence of dualities in Figure \ref{pic:4pt:seib} (depicted also in Figure \ref{fig:an:4pt} in a more collapsed way)  implies that conjugating one pair of minimal/maximal punctures moment maps (by introducing flip fields) to make them of the same type, the two minimal punctures and the two maximal ones appear exactly on the same footing. We expect that same type of punctures should be exchangeable by duality arguments \cite{Razamat:2020bix}, and here they are manifestly so. The model flows to a point on the conformal manifold which is invariant under the exchange of the punctures. Moreover since the superpotential distinguishing all the punctures is the irrelevant baryonic one there is no actually a direction on the conformal manifold preserving all the symmetries we want. 
However when we will glue these theories together in principle a conformal manifold can arise.\footnote{The situation is very similar to what happens in the discussion of the compactification of the minimal $\SU(3)$ SCFT \cite{Razamat:2018gro}.} The issue is that for low enough number of punctures/``small'' enough punctures/ low genus/low flux some general expectations (such as existence of exactly marginal deformations corresponding to complex structure moduli) from the 4d theory might fail. 

%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.3\linewidth]{figures/d4trinion.pdf}\;\;\;\;\;
                \includegraphics[width=0.6\linewidth]{figures/d4genus3.pdf}
        \caption{On the left we have the three punctured sphere, two maximal $\SU(3)$ punctures and one maximal $\USp(4)$ puncture, with zero flux of the $(D_5,D_5)$ minimal conformal matter theory. The theory has baryonic superpotentials consistent with the assigned charges.  The superpotential is built by taking a triplet of fundamentals transforming under one of the $\SU(3)$s, computing third antisymmetric power to build a singlet of the $\SU(3)$, and then taking  the fields transforming under $\USp(4)$ to the second antisymmetric power to build a singlet under it. This superpotential is irrelevant for the trinion. On the right hand side we glue four trinions into a genus three surface. This theory has the baryonic superpotentials as well as the ones corresponding to closed loops in the quiver which are consistent with the charges.
        The symmetry of the theory is $\SU(10)\times \U(1)_h\subset \SO(20)$ where $\SO(20)$ is the symmetry of the 6d SCFT.}
        \label{pic:trinionAndgenus3D4}
\end{figure}
%%%%%%%%%%%%%


Moreover there is another way to view this theory. As was argued in \cite{Razamat:2019ukg,Razamat:2020bix} in general we expect that the $\SU(2)$ punctures might combine into  a bigger puncture of $\USp$ type. The $\SU(2)$ punctures are obtained by partial closing of the $\USp(2N)$ puncture. These partial closings are obtained by giving vevs to some components of the moment map (with addition of certain flip fields) and the symmetry can be broken to $\USp(2k)$ with $k<N$. The claim of \cite{Razamat:2019ukg,Razamat:2020bix} is that if we have $k\leq N$ minimal $\SU(2)$ punctures somewhere on the conformal manifold of the theory they might recombine into an $\USp(2k)$ puncture. Thus for $N>1$ we can view the theories of Figure  \ref{fig:an:4pt} alternatively as a three punctured sphere with two maximal $\SU(N+1)$ punctures and a non maximal/minimal $\USp(4)$ puncture. Note again that this symmetry is trivially manifest in the Lagrangian and is preserved by the irrelevant baryonic deformation.

For the special case of $N=2$ the $\USp(4)$ puncture is a maximal one. Thus this new description discussed here  gives us a completely Lagrangian formulation of a sphere with three maximal punctures in this case. Since we obtain this theory by S-gluing two copies of identical theories the flux associated to it is zero.
 Starting from this sphere we can explicitly build theories corresponding to arbitrary surfaces. For example, in Figure \ref{pic:trinionAndgenus3D4}
a genus three surface with zero flux is depicted. Doing so all the deformations (including the baryonic ones) become relevant/exactly marginal. In particular we can compute say the index of the genus $g$ theory and obtain,
\be
{\cal I}=1+q\,p\,\left(3g-3+(g-1)\, (1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6})\right)+\cdots\,.
\ee which is exactly as expected \cite{babuip}. Note that,
\be
1+{\bf 99}_{\SU(10)}+{\bf 45}_{\SU(10)}\, h^6+\overline {\bf 45}_{\SU(10)}\, h^{-6}\;\;\;\to\;\;\;\; {\bf 190}_{\SO(20)}\,,
\ee using the  decomposition of $\SO(20)$ into irreps of $\SU(10)\times \U(1)$. The symmetry of the 6d theory is $\SO(20)$ and as the flux is zero we expect to see it appear somewhere on the conformal manifold.





==> sections/comments_cn_a1n.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Comments on $C_N$ and $A_1^{\otimes N}$ generalizations}
\label{sec:comments:CNA1N}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Additional puncture for higher rank van Diejen


%%%%%%%%%%%%
\begin{figure}[!btp]
        \centering
        \includegraphics[width=0.6\linewidth]{figures/affineddynkin.pdf}
        \caption{ Upon a circle compactification of the non minimal $(D,D)$ conformal matter, $k$ M5 branes probing $D_{N+3}$ singularity, with proper holonomies turned on one obtains a 5d effective quiver description shaped as the affine Dynkin diagram of $D_{N+3}$ with $SU(k)$ and $SU(2k)$ gauge groups as depicted here. Upon compactification to four dimensions this five dimension description gives a puncture with symmetry $SU(k)^2\times SU(2k)^N\times SU(k)^2$ with a pattern of moment map operators corresponding to the Dynkin diagram.}
        \label{pic:affineDDynkin}
\end{figure}
%%%%%%%%%%%%%




